Viscometry of electron fluids from symmetry

When electrons flow as a viscous fluid in anisotropic metals, the reduced symmetry can lead to exotic viscosity tensors with many additional, nonstandard components. We present a viscometry technique that can, in principle, measure the multiple dissipative viscosities allowed in isotropic and anisotropic fluids alike. By applying representation theory to exploit the intrinsic symmetry of the fluid, our viscometry is also exceptionally robust to both boundary complications and ballistic effects. We present the technique via the illustrative example of dihedral symmetry, relevant in this context as the point symmetry of 2D crystals. Finally, we propose a present-day realizable experiment for detecting, in a metal, a novel hydrodynamic phenomenon: the presence of rotational dissipation in an otherwise isotropic fluid.

==> coverletter.tex <==
Dear Editor,	

Attached is our manuscript "Viscometry of electron fluids from symmetry", submitted as a Letter to Physical Review Letters.

Hydrodynamics is perhaps one of the oldest scientific pursuits, arguably dating back to Archimedes in about 250 BC. Indeed, hydrodynamics finds application in many diverse and modern fields of physics, including atmospheric physics, liquid crystals, quark-gluon plasma and -- most recently -- electrons in ultra-pure materials. 

In the existing electron hydrodynamics literature, much attention has been focused on how relatively ordinary fluid phenomena can have interesting implications when realized in a metal, e.g. whirlpools leading to negative non-local resistance in graphene. In this work, we further open the rapidly growing field of electron hydrodynamics by, for the first time, inverting this paradigm. In this work, we explain how to discover, in anisotropic electron fluids, a new hydrodynamic phenomenon: the presence of viscous resistance to rigid rotations, as an isolated correction to an otherwise-isotropic fluid.

From the macroscopic perspective, the appearance of rotational viscosity at all is rather striking. When a fluid is subject to a rigid rotation, there is no relative motion within the fluid, yet rotational viscosity nevertheless predicts internal viscous resistance. Moreover, the heat dissipated through rotational viscosity is localized in space to the center of the rigid rotation, where the fluid is completely stationary. 

%[delete] It has been traditionally believed that rotational viscosity necessarily requires that the fluid particles themselves have rotational degrees of freedom; for this reason, the only previous discussion of rotational viscosity of which we are aware has been restricted to the context of liquid crystal physics. 

%[delete] Even for free liquid crystals (LCs), however, the rotational viscosity is not a true hydrodynamic coefficient. This is because, when free LCs break rotational invariance, they only do so spontaneously. This means angular momentum is still conserved, and hence the fluid does not allow for a viscosity component that would couple to an antisymmetric stress tensor component (i.e. the rotational viscosity). Alternatively, one may explicitly break rotational invariance in LCs by applying an in-plane magnetic field, and while this does in fact generate rotational viscosity, many other viscosities will also appear due to the simultaneous loss of many other symmetries (including time-reversal invariance).

Electronic excitations in a metal generically exhibit this effect simply by virtue of living entirely within the context of an ionic lattice, which explicitly breaks rotational symmetry. For hexagonal metals in particular, we predict that rotational viscosity will appear in an isolated way, joined only by the two isotropic transport coefficients (bulk and shear viscosity) present in any standard fluid. Utilizing mathematical techniques from the linear representation theory of finite groups, we further propose a ``smoking gun” experiment to discover the isolated presence of rotational viscosity in hexagonal electron fluids (e.g. trilayer graphene and/or PdCoO2), which we go on to show is easily within reach of present-day experiments. 

Finally, we argue in the Letter that our proposal is in fact the only straightforward way rotational viscosity of electrons can hope to be detected.  The detection of rotational viscosity would represent the first qualitatively new phenomenon that is easiest to see in an electronic fluid.  To re-iterate: until now, hydrodynamic electrons have been understood via textbook Navier-Stokes equations with zero additional structure.  The discovery of rotational viscosity, whose origin is most crisply illustrated by anisotropic electron fluids, would represent a contribution of the "electrons" literature to "hydrodynamics".

[i tried to shorten the lC discussion but still unhappy...] Rotational viscosity has been overlooked in the modern (condensed matter) literature.  The closest analogues arising in (pinned) liquid crystals.  However in these settings, there are both internal rotational dynamics and (in the case of pinning by magnetic fields) broken time-reversal symmetry.  Only the electronic setting allows for the clean identification of rotational viscosity without the additional complications of extreme anisotropy or unnecessary broken symmetry.  

Beyond providing a concrete experimental roadmap to the detection of rotational viscosity, our mathematical results suggest a novel viscometry technique for fluids (electronic or otherwise) of known point group symmetry. Representation theory allows us to (a) predict all the viscosity components that will generically appear, and (b) propose device geometries that isolate their dissipative effects in a robust way, so that all said viscosity components can in principle be measured. This of course implies that our viscometry is also applicable to the study of shear (and possibly even bulk) viscosity of isotropic electron fluids, which remain of great interest.

By contrast, existing viscometry techniques for electron fluids are indirect and, as they assume isotropy, will in general return a complicated, inseparable mixture of viscosity components when applied in metals of lower symmetry. Even for isotropic fluids, where both existing techniques and our proposed viscometry are in principle applicable, our technique has the further advantage of being exceptionally robust to boundary complications and ballistic effects, both of which have traditionally hampered metrology of electron fluids. For this reason, we believe our Letter satisfies PRL’s "Introduce new techniques or methodologies with significant impact" criterion.

Our results provide both relevant theory for and path towards experimental discovery of a novel hydrodynamic phenomenon.  Therefore, we expect that they will be of broad interest, especially given the exciting and experimentally-realizable context where such a discovery can be made. For these reasons, we believe our Letter additionally satisfies PRL’s "Be of unusual intrinsic interest to PRL's broad audience" criterion.

Sincerely,

Caleb Q. Cook
Andrew Lucas

